Tracing Chemical Depletion in Evolved Binaries Hosting Second-Generation Transition Discs

The mechanisms responsible for chemical depletion across diverse astrophysical environments are not yet fully understood. In this paper, we investigate chemical depletion in post-AGB/post-RGB binary stars hosting second-generation transition discs using high-resolution optical spectra from HERMES/Mercator and UVES/VLT. We performed a detailed chemical abundance analysis of 6 post-AGB/post-RGB stars and 6 post-AGB/post-RGB candidates with transition discs in the Galaxy and in the Large Magellanic Cloud. The atmospheric parameters and elemental abundances were obtained through 1D LTE analysis of chemical elements from C to Eu, and 1D NLTE corrections were incorporated for elements from C to Fe. Our results confirmed that depletion efficiency, traced by the [S/Ti] abundance ratio, is higher in post-AGB/post-RGB binaries with transition discs compared to the overall sample of post-AGB/post-RGB binaries. We also examined correlations between derived abundances and binary system parameters (astrometric, photometric, orbital, pulsational). Additionally, we compared the depletion patterns in our sample to those observed in young stars with transition discs and in the interstellar medium. We confirmed that the depletion is significantly stronger in post-AGB/post-RGB binaries with transition discs than in young stars with transition discs. Furthermore, we found that [X/Zn] abundance ratio trends of volatile and refractory elements in post-AGB/post-RGB binaries with transition discs generally resemble similar trends in the interstellar medium (except for trends of [Si/Zn] and [Mg/Zn] ratios). These findings, although based on a limited sample, provide indirect constraints for depletion mechanism in circumbinary discs around post-AGB/post-RGB stars.

==> Figures/TEXs/FigAAllCmp.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=.41\linewidth]{Figures/PDFs/Comp/DepletionComparCTOri1.pdf}
    \includegraphics[width=.41\linewidth]{Figures/PDFs/Comp/DepletionComparSTPup2.pdf}
    \includegraphics[width=.41\linewidth]{Figures/PDFs/Comp/DepletionComparRUCen3.pdf}
    \includegraphics[width=.41\linewidth]{Figures/PDFs/Comp/DepletionComparACHer4.pdf}
    \includegraphics[width=.41\linewidth]{Figures/PDFs/Comp/DepletionComparADAql5.pdf}
    \includegraphics[width=.41\linewidth]{Figures/PDFs/Comp/DepletionComparEPLyr6.pdf}
    \caption{Elemental abundances of transition disc stars -- CT Ori (\#1), ST Pup (\#2), RU Cen (\#3), AC Her (\#4), AD Aql (\#5), EP Lyr (\#6) -- as functions of condensation temperature \citep{lodders2003CondensationTemperatures, wood2019CondensationTemperatures}. The legend for the symbols and colours used is included within the plot.}\label{figA:allcmp1}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=.41\linewidth]{Figures/PDFs/Comp/DepletionComparDYOri7.pdf}
    \includegraphics[width=.41\linewidth]{Figures/PDFs/Comp/DepletionComparAFCrt8.pdf}
    \includegraphics[width=.41\linewidth]{Figures/PDFs/Comp/DepletionComparGZNor9.pdf}
    \includegraphics[width=.41\linewidth]{Figures/PDFs/Comp/DepletionComparV1504Sco10.pdf}
    \includegraphics[width=.41\linewidth]{Figures/PDFs/Comp/DepletionComparLMCV077011.pdf}
    \includegraphics[width=.41\linewidth]{Figures/PDFs/Comp/DepletionComparLMCV315612.pdf}
    \caption{Elemental abundances of transition disc candidates -- DY Ori (\#7), AF Crt (\#8), GZ Nor (\#9), V1504 Sco (\#10), LMC V0770 (\#11), LMC V3156 (\#12) -- as functions of condensation temperature \citep{lodders2003CondensationTemperatures, wood2019CondensationTemperatures}. The fit of LTE abundances is denoted with solid black line and the fit of NLTE-corrected abundances is denoted with dashed red line. Turn-off temperature $T_{\rm turn-off}$ denotes the break (in case of two-piece linear fit) or is set as 600 K (in case of one-piece linear fit). Depletion rate $\nabla_{\rm 100K}$ denotes the rate of linear decrease in the profile fits per 100~K.}\label{figA:allcmp2}
\end{figure*}

==> Figures/TEXs/FigOneSED.tex <==
\begin{figure}
    \centering
    \includegraphics[width=1.09\linewidth]{Figures/PDFs/SEDs/IRAS06034+1354SED.png}
    \caption{SED of DY Ori (\#7) (see Section~\ref{ssec:dobpht}). The red solid line is the appropriate Kurucz model atmosphere fitted to the data. The black solid line is the scaled de-reddened model atmosphere. The integration of de-reddened model atmosphere provides the SED luminosity (see Section~\ref{ssec:doblum}). The legend for the symbols and colours used are included within the plot (for all SEDs, see Appendix~\ref{app:sed}).}\label{fig:oneSED}
\end{figure}

==> Tables/TableANLTTst.tex <==
\begin{table}
    \centering
    \caption{First-iteration NLTE atmospheric parameters of the transition disc sample (see Appendix~\ref{app:nlt} for more details).}\label{tabA:nlttst}
    \begin{tabular}{|c@{\hspace{0.001cm}}|c@{\hspace{0.001cm}}|c@{\hspace{0.001cm}}|c@{\hspace{0.001cm}}|c@{\hspace{0.001cm}}|c@{\hspace{0.001cm}}|} \hline
        ID & Name & $T_{\rm eff}$ & $\log g$ & $[$Fe/H$]$ & $\xi_{\rm t}$ \\ \hline
        1 & CT Ori & 6710$\pm$90 & 3.17$\pm$0.14 & --1.17$\pm$0.17 & 5.47$\pm$0.06 \\
        2 & ST Pup & 5440$\pm$70 & 1.16$\pm$0.11 & --1.71$\pm$0.08 & 5.17$\pm$0.07 \\
        3 & RU Cen & 6420$\pm$90 & 3.03$\pm$0.15 & --1.45$\pm$0.10 & 5.11$\pm$0.13 \\
        4 & AC Her & 6650$\pm$100 & 3.22$\pm$0.12 & --0.90$\pm$0.12 & 5.54$\pm$0.11 \\
        5 & AD Aql & 6860$\pm$130 & 4.05$\pm$0.18 & --1.45$\pm$0.12 & 5.51$\pm$0.33 \\
        6 & EP Lyr & 6600$\pm$110 & 3.03$\pm$0.17 & --1.49$\pm$0.21 & 3.80$\pm$0.04 \\ \hline
        7 & DY Ori & 7000$\pm$140 & 3.82$\pm$0.27 & --1.19$\pm$0.09 & 3.90$\pm$0.11 \\
        8 & AF Crt & 5690$\pm$160 & 1.01$\pm$0.33 & --2.45$\pm$0.10 & 4.87$\pm$0.21 \\
        9 & GZ Nor & 4890$\pm$90 & 0.59$\pm$0.14 & --1.83$\pm$0.09 & 9.96$\pm$0.60 \\
        10 & V1504 Sco & 6820$\pm$80 & 3.25$\pm$0.10 & --0.31$\pm$0.17 & 4.66$\pm$0.03 \\
        11 & LMC V0770 & 5640$\pm$260 & 0.78$\pm$0.32 & --2.49$\pm$0.12 & 3.69$\pm$0.12 \\
        12 & LMC V3156 & 6390$\pm$820 & 3.00$\pm$0.61 & --2.10$\pm$0.05 & 31.39$\pm$200 \\ \hline
    \end{tabular}
\end{table}
